A Twin Neural Model for Uplift

Uplift is a particular case of conditional treatment effect modeling. Such models deal with cause-and-effect inference for a specific factor, such as a marketing intervention or a medical treatment. In practice, these models are built on individual data from randomized clinical trials where the goal is to partition the participants into heterogeneous groups depending on the uplift. Most existing approaches are adaptations of random forests for the uplift case. Several split criteria have been proposed in the literature, all relying on maximizing heterogeneity. However, in practice, these approaches are prone to overfitting. In this work, we bring a new vision to uplift modeling. We propose a new loss function defined by leveraging a connection with the Bayesian interpretation of the relative risk. Our solution is developed for a specific twin neural network architecture allowing to jointly optimize the marginal probabilities of success for treated and control individuals. We show that this model is a generalization of the uplift logistic interaction model. We modify the stochastic gradient descent algorithm to allow for structured sparse solutions. This helps training our uplift models to a great extent. We show our proposed method is competitive with the state-of-the-art in simulation setting and on real data from large scale randomized experiments.

==> figures/alpha.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/fig/Qini_alpha_valid_IE.jpg}
    \includegraphics[width=0.45\textwidth]{figures/fig/Qini_alpha_valid_TO.jpg}
    \caption{Fine-tuning of the trade-off constant $\alpha$ on the Canadian insurer dataset. The left curve corresponds to the (IE) loss and the right one to the (TO) loss. }
    \label{fig:alphaie}
\end{figure}

==> figures/framework.tex <==
\begin{figure}[!h]
    \centering
    \begin{tikzpicture}
    
    \tikzset{dist/.style={path picture= {
    \begin{scope}[x=1pt,y=10pt]
      \draw plot[domain=-6:6] (\x,{1/(1 + exp(-\x))-0.5});
    \end{scope}
    }}}
    \tikzstyle{sigmoid}=[draw,fill=gray!50,circle,minimum size=20pt,inner sep=0pt,dist]
    
    \filldraw[fill=gray!20!white, draw=black]  (0,0) rectangle (0.5,2);
    \node at (-0.25,1) {$\x$};
    \filldraw[fill=gray!10!white, draw=black] (0,-0.75) rectangle (0.5,-0.25); 
    \node at (0.25,-0.5) {$\mathbf{1}$};

    \filldraw[fill=blue!10!white, draw=black] (0,-1.5) rectangle (0.5,-1); 
    \node(treatment) at (-0.25,-1.25) {$t$};
    
    \filldraw[fill=gray!20!white, draw=black] (0,-3.75) rectangle (0.5,-1.75);
    \node at (-0.25,-2.75) {$\x$};
    \filldraw[fill=gray!10!white, draw=black] (0,-4.5) rectangle (0.5,-4); 
    \node at (0.25,-4.25) {$\mathbf{0}$};

    \filldraw[fill=gray!20!white, draw=black] (1,-0.75) rectangle (1.5,2);
    \node at (1.25,0.75) {$h_1$};
    \draw [->] (0.6,0.75) -- (0.9,0.75);
    
    \filldraw[fill=gray!20!white, draw=black] (1,-4.5) rectangle (1.5,-1.75);
    \node at (1.25,-3) {$h_1$};
    \draw [->] (0.6,-3) -- (0.9,-3);
    
    
    %\filldraw[fill=gray!20!white, draw=black] (1.75,-4.5) rectangle (3.25,-1.75);
    \node at (2.5,-3) {$\ldots\boldsymbol{\theta}\ldots$};
    
    %\filldraw[fill=gray!20!white, draw=black] (1.75,-0.75) rectangle (3.25,2);
    \node at (2.5,0.75) {$\ldots\boldsymbol{\theta}\ldots$};

    \filldraw[fill=gray!20!white, draw=black] (3.5,-0.75) rectangle(4,2);
    \node(lp1) at (3.75,0.75) {$h_L$};
    
    \filldraw[fill=gray!20!white, draw=black] (3.5,-4.5) rectangle (4,-1.75);
    \node(lp0) at (3.75,-3) {$h_L$};
    
    \node (p1)[sigmoid] at (5, 0.75) {};
    \node (p0)[sigmoid] at (5, -3) {};
    
    \filldraw (5,-1.25) circle (3pt);
    \draw [->] (0.5,-1.25) -- (5,-1.25);
    
    \draw[thick] (lp1) -- (p1) node [midway,above=-0.06cm] {};
    \draw[thick] (p1) -- (p0) node [midway,above=-0.06cm] {};
    \draw[thick] (lp0) -- (p0) node [midway,above=-0.06cm] {};
    
    \node(mu) at (4.7,-0.2) {$\mu_1$};
    \node(mu) at (4.7,-2) {$\mu_0$};
    \draw [->] (5,-1.25) -- (6.25,-1.25);
    \draw  (5.35,-3) -- (5.85,-3);
    \draw  (5.85,-3) -- (5.85,-1.5);
    \draw  (5.85,-1.5) -- (5.65,-1.5);
    \draw  (5.65,-1.5) -- (5.65,-1);
    \draw  (5.65,-1) -- (5.85,-1);
    \draw  (5.85,-1) -- (5.85,0.35);
    \draw [->] (5.85,0.35) -- (6.25,0.35);
    \draw [->] (5.35,0.75) -- (6.25,0.75);
    
    %\node(mut) at (5.35,-1.1) {$\mu_t$};
    
    \filldraw[fill=gray!15!white, draw=black] (6.3,-1.6) rectangle (7.5,-0.9);
    %\node at (6.9,-1.25) {$\mathcal{L}_{\boldsymbol{\theta}}(\mu_t)$};
    \node at (6.9,-1.25) {$\mu_t$};
    
    \filldraw[fill=gray!15!white, draw=black] (6.3,0.2) rectangle (7.5,0.9);
    %\node at (7.07,0.5) {$\mathcal{J}_{\boldsymbol{\theta}}(\mu_0,\mu_1)$};
    \node at (6.9,0.55) {$\mu_1-\mu_0$};
    
    \end{tikzpicture}
    \caption{SMITE neural network architecture.}
    \label{fig:nite}
\end{figure}


==> figures/losses.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/fig/to_loss.jpg}
    \includegraphics[width=0.45\textwidth]{figures/fig/ie_loss.jpg}
    \caption{Uplift regularization functions learning curves:  direct $\mathcal{J}$ (left) and indirect $\mathcal{I}$ (right).}
    \label{fig:instabilty}
\end{figure}

==> figures/uplift_evolutions.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/fig/Distribution_Uplift.jpg}
    \includegraphics[width=0.45\textwidth]{figures/fig/Bad_Distribution.jpg}
    \caption{Predicted uplift distributions on real data. We show evolution as the number of epochs increases. (left): For {\it IE}, individual uplifts are pushed away from zero and cover a small range within the interval $[0.000; 0.016]$ as training goes on. (right): {\it Logistic} model. The range covered grows as the number of epochs increases and stays more or less centered at $0$. The final interval is about $[-0.02,0.03]$. That behaviour is associated with overfitting.}
    \label{fig:pred_uplift_evol}
\end{figure}

==> old_tex/experiments.tex <==
\newpage
\section{Old Experiments Section}

%We conduct a simulation study to examine the performance of our models. We compare with existing uplift methods using three types of datasets: i) a real-world dataset from a marketing campaign (see Section~\ref{sec:application} for the analysis); ii) bootstrapped versions of the real-world dataset with synthetic outcomes generated from tree-based models, and iii) synthetic datasets generated from parametric models.

\subsection{Fine-tuning}

Deep Learning has enabled remarkable progress over the last years on a variety of tasks, such as image recognition, speech recognition, and machine translation. One crucial aspect for this progress are novel neural architectures. Currently employed architectures have mostly been developed manually by human experts, which is a time-consuming and error-prone process. Because of this, there is growing interest in automated neural architecture search (NAS) methods. NAS methods can be categorized according to three dimensions \citep{elsken2018neural}: search space, search strategy, and performance estimation strategy.

The search space defines which architectures can be represented
in principle. Incorporating prior knowledge about typical properties of architectures well-suited for a task can reduce the size of the search space and simplify the search. SMITE architecture is a Sieamese multi-layer perceptron. Therefore, the search space for the architecture is first defined by the number of hidden layers and the number of hidden units per layer. However, it should not be limited to these two parameters. The choice of loss functions, regularization and activations in deep networks has also a significant effect on the training dynamics and task performance. These functions are therefore part of the architecture and should be included in the search space.

Neural network activations determine the output of a node and are a crucial component of deep learning. When the activation function is non-linear, then a two-layer neural network can be proven to be a universal function approximator. The identity activation function does not satisfy this property. When multiple layers use the identity activation function, the entire network is equivalent to a single-layer model. The Parameteric Rectified Linear Unit (PReLU) \citep{he2015delving} has been proposed as an extension of Rectified Linear Unit (ReLU) \citep{nair2010rectified} in order to improve image classification accuracy. The PReLU function is defined as

\[
f_a (x) = 
\begin{cases}
    x, ~\mathrm{if}~ x \geq 0\\
    ax, ~\mathrm{otherwise}
\end{cases}
\]

where $a \in [0;1]$ is learned in the training via backpropagation. When $a=0$, PReLU simplifies to ReLU and if $a$ is set to a fixed value, PReLU simplifies to Leaky ReLU (LReLU)  \citep{maas2013rectifier}.


The search strategy details how to explore the search space
(which is often exponentially large or even unbounded). It encompasses the classical exploration-exploitation trade-off since, on the one hand, it is desirable to find well-performing architectures quickly, while on the other hand, premature convergence to a region of suboptimal architectures should be avoided. In \cite{yang2019evaluation},  based on a benchmark of 8 NAS methods on 5 datasets, they compare methods with different search spaces, using a method’s relative improvement over the randomly sampled average architecture, which effectively removes advantages arising from expertly engineered search spaces or training protocols. Surprisingly, they find that many NAS techniques struggle to significantly beat the average architecture baseline. Furthermore, it is desirable to have a search strategy because unfortunately, in many deep learning tasks, training is computationally expensive. However, for our application, training SMITE on the real data takes 10 minutes for 100 epochs (on a Dual Intel Xeon 256 Gb RAM and 1 Titan V12GB). Therefore, we believe that grid search is suitable for SMITE architecture search. Table~\ref{tab:NAS} summarizes the hyper-parameters responsible for defining the architecture of SMITE. Hyper-parameter 3 must be defined for each layer. Although hyper-parameters 5-6 do not modify the architecture, they are important in terms of training. We prefer to enumerate them in Table~\ref{tab:NAS} in order to include them in the architecture search. Hyper-parameter 7 is important for reproducible results. Our experimental results are presented in Table~\ref{tab:experiments_low_rank_full_rank} on the real-world marketing campaign dataset (see Section~\ref{sec:application} for the description).

\begin{table}[htb]
    \caption{Hyper-parameters that define the architecture of SMITE.}
    \centering
    \begin{tabular}{|c||l|l|l|}
         \hline
         \# &  Hyper-parameter & Type & Scope\\
         \hline
         1 & \# of hidden layers & Integer & $\{0,1\}$\\
         2 & \# of hidden units & Integer & $\{8, 16, 32, 64, \ldots, 2048\}$\\
         3 & Activation & Nominal & $\{$ReLU, LReLU$(0.05)\}$\\
         4 & Objective function & Nominal & $\{$TO, IE$\}$ \\
         5 & Batch size $m$ & Integer & $\{128,256\}$ \\
         6 & Learning rate $\xi$ & Continuous & $\{0.01,0.02,\ldots,0.10\}$ \\
         7 & Seed & Integer & $\{1,2,3,\ldots,10\}$ \\
         \hline
    \end{tabular}
    \label{tab:NAS}
\end{table}

The objective of NAS is typically to find architectures that achieve high predictive performance on unseen data. Performance estimation refers to the process of estimating this performance: the simplest option is to perform a standard training and validation of the architecture on data. Here, we use the reference metric for uplift, that is, the adjusted Qini coefficient \eqref{eq:qadj}.


\begin{table}[H]
    \centering
    \caption{Fine-tuning SMITE with $p=40$ using the insurance policy data. Reported $\qadj$ are averaged over $30$ runs on validation sets, with standard errors in parenthesis. Here, the objective function used is IE.}
    \begin{tabular}{|c||l|l|l|l|}
        \hline
        $m$ &  No SVD & $r=\min\{m,p\}$ & $r=\ceil{0.5\min\{m,p\}}$ & $r=\ceil{0.1\min\{m,p\}}$\\
        \hline
        8 & & & & \\
        16 & & & & \\
        32 & & & & \\
        64 & & & & \\
        128 & & & & \\
        256 & & & & \\
        512 & & & & \\
        1024 & & & & \\
        2048 & & & & \\
        \hline
    \end{tabular}
    \label{tab:experiments_low_rank_full_rank}
\end{table}



\subsection{Data generation}

We evaluate the performance of SMITE using synthetic data generated using two types of mechanisms.

\paragraph{Bootstrap Data.} The underlying treatment effects are inaccessible in real-world data. To create realistic scenarios, we based one of our simulation study data generation on insurance policy data. Moreover, since we compare SMITE to random forests, we want to evaluate its performance when the data generation process comes from a tree-based model. We follow the procedure in the simulation studies of \cite{belba2019qbased}. These simulations allow us to evaluate if SMITE can recover the right representation for data generated from a tree-based model. This also makes comparisons to random forest methods fair.

Several tree-based methods have been suggested in the uplift literature. Here, we use the uplift random forest as the data generation process, which is readily available in the {\bf R} library {\it uplift} \citep{guelman2014R_uplift}. We fit the random-forest on a random sub-sample $\mathcal{D}$ of the real data. We use $100$ trees and the Kullback-Leibler split criterion. Each tree has maximum depth of $5$. Based on the fitted model, we can extract the probabilities $\mu_0(\x)$ and $\mu_1(\x)$ for any given value $\mathbf{x}$. We use these probabilities to draw synthetic outcomes for treated and control observations. We start by creating a bootstrap sample $\mathcal{S}$ of size $n_\mathcal{S}$ from $\mathcal{D}$. For each observation $\mathbf{x}_i \in \mathcal{S}$, we generate a random vector $\tilde{y}_i =(\tilde{y}_{i0}, \tilde{y}_{i1})$, where $\tilde{y}_{i0}$ is the binary outcome of a Bernoulli trial with success probability $\mu_0(\mathbf{x}_i)$, and  $\tilde{y}_{i1}$ is the binary outcome of a Bernoulli trial with success probability  $\mu_1(\mathbf{x}_i)$, $i=1,\ldots, n_\mathcal{S}$. The augmented synthetic dataset $\{ \x_i , t_i, \tilde{y}_i \}_{i=1}^{n_{\mathcal{S}}}$ is the data of interest in the simulation.

We repeat this process several times. Each bootstrapped data size is $10,000$ observations with $40$ covariates. 




\subsection{Experimental results}

For both simulated datasets, we do not consider any out-of-sample subset. In Monte Carlo settings, we are able to generate as much data as we want. Therefore, we first fine-tuned the methods on a single synthetic dataset of same size as the one we used in the repeated simulations presented. We generate $n=10,000$ observations with $p=40$ covariates for the bootstrapped data. For the fully synthetic datasets, we report results from experiments with $n=10,000$ observations and $p=100$ covariates. We split into training and validation and compare the results averaged over $30$ runs for the models that performed best on the validation set. 

Results are described in Table \ref{tab:boot_perf} for the bootstrap datasets and Table \ref{tab:synthe_perf} for the synthetic datasets. For the fully synthetic data, we see that Causal Forest (H) and SMITE (TO) had similar performance on the validation set while SMITE (IE) significantly outperformed all the other methods. For the bootstrap data for which the outcomes were generated based on random forest model, it is interesting to see that SMITE (TO) and Causal Forest (H) give similar results. Moreover, once again, the SMITE (IE) model outperforms all the other models.

%bootstrap data results
\input{tables/table_bootstrap.tex}

%MOULOUD
%\textcolor{blue}{HERE WE NEED TO SHOW ESTIMATED AND PREDICTED UPLIFTS DISTRIBUTIONS PER METHOD. I THINK THIS WILL SHOW THAT RF METHODS COVER A RANGE THAT IS A LOT LARGER THAN SMITE. WE CAN ALSO COMPUTE THE EMPIRICAL VARIANCES AND COMPUTE A CONFIDENCE INTERVAL FOR THE VARIANCE OF THE PREDICTED UPLIFTS TO SEE IF THERE ARE SIGNIFICANTLY LARGER THANT SMITE'S VARIANCE.}


%synthtetic data results
\input{tables/table_synthetic.tex}


==> others/experiements_old.tex <==

\section{Experiments}
\label{sec:appendix_experiments}


In this section, we present in more detail the experimental protocol as well as the results associated with the different scenarios.


Each simulation is defined by a data-generating process with a known effect function. Each run of each simulation generates a dataset, and split into training, validation, and test subsets. We use the training data to estimate $L$ different uplift functions $\{\hat{u}_l\}_{l=1}^L$ using $L$ different methods. For each of those we calculate the validation metric $\qadj$ using the data in validation set. The models selected by optimizing each validation-set metric are then used to predict the uplift on the test set.

\paragraph{Data generating process}

We generate synthetic data similar  to  \cite{powers2018some}. For each experiment, we generate $n$ observations and $p$ covariates. We draw odd-numbered covariates independently from a standard Gaussian distribution. Then, we draw even-numbered covariates independently from a Bernoulli distribution with probability $1/2$. Across all experiments, we define the mean effect function $\mu(\cdot)$ and the treatment effect function $\tau(\cdot)$ for a given noise level $\sigma^2$. Given the elements above, our data generation model is, for $i=1,...,n$,
\begin{align*}
    &Y_i^* \mid \x_i, t_i \sim \mathcal{N}(\mu(\x_i) + t_i\tau(\x_i), \sigma^2),\\
    &Y_i = \mathbbm{1}(Y_i^* > 0 \mid \x_i, t_i)
\end{align*}
where $t_i$ is the realisation of the random variable $T_i \sim \mathrm{Bernoulli}(1/2)$ and $Y_i$ is the binary outcome random variable. Therefore, $Y_i$ follows a Bernoulli distribution with parameter $\mathrm{Pr}(Y_i^* > 0 \mid \x_i, t_i)$ and it is easy to recover the ``true'' uplift $u_i^*$, that is,
\begin{align}
    u_i^* &= \mathrm{Pr}(Y_i^* > 0 \mid \x_i, T_i = 1) - \mathrm{Pr}(Y_i^* > 0 \mid \x_i, T_i = 0) \nonumber \\
    u_i^* &= \Phi \Bigl( \frac{\mu(\x_i) + \tau(\x_i)}{\sigma} \Bigr) - \Phi \Big( \frac{\mu(\x_i)}{\sigma} \Big) \label{eq:sim_true_uplift}
\end{align}
for $i=1,\ldots,n$, where $\Phi(.)$ is the standard Gaussian cumulative distribution function.

Following \cite{powers2018some},  within each set of simulations, we make different choices of mean effect function and treatment effect function, each represents a wide variety of functional forms, univariate and multivariate, additive and interactive, linear and  piecewise constant. The functions are
\begin{align*}
    f_1(\x) &= 0 \\
    f_2(\x) &= 5 \mathbbm{1}(x_1 > 1) - 5\\
    f_3(\x) &= 2 x_1 - 4 \\
    f_4(\x) &= x_2 x_4 x_6 + 2 x_2 x_4 (1-x_6) +3x_2(1-x_4)x_6 + 4x_2(1-x_4)(1-x_6) + 5(1-x_2)x_4x_6 \\
            &+ 6(1-x_2)x_4(1-x_6) + 7 (1-x_2)(1-x_4)x_6 + 8(1-x_2)(1-x_4)(1-x_6)\\
    f_5(\x) &= x_1 + x_3 + x_5 + x_7 + x_8 + x_9 - 2\\
    f_6(\x) &= 4 \mathbbm{1}(x_1 > 1)\mathbbm{1}(x_3 > 0) + 4\mathbbm{1}(x_5 > 1)\mathbbm{1}(x_7 > 0) + 2x_8x_9\\
    f_7(\x) &= \frac{1}{2} (x_1^2 + x_2 + x_3^2 + x_4 + x_5^2 + x_6 + x_7^2 + x_8 + x_9^2 - 11)\\
    f_8(\x) &= \frac{1}{\sqrt{2}} (f_4(\x) + f_5(\x)).
\end{align*}

Table~\ref{tab:scenarios} gives the mean and treatment effect functions for the different randomized simulations, in terms of the eight functions above. In Figure~\ref{fig:qini_curves_scene}, we show the Qini curves associated with the ``true" uplift $u^*$. 


\begin{table}[!ht]
    \centering
    \caption{Specifications for the 5 simulation scenarios. The rows of the table correspond, respectively, to the sample size, dimensionality, mean effect function, treatment effect function and noise level.}
    \label{tab:scenarios}
    \begin{tabular}{l|ccccc}
        Scenarios & 1 & 2 & 3 & 4 & 5\\
        Parameters & & & & & \\
        \hline
        $n$ & 10000 & 20000 & 20000 & 20000 & 20000 \\
        $p$ & 200 & 100 & 100 & 100 & 100 \\
        $\mu(\x)$ & $f_7(\x)$ & $f_3(\x)$ & $f_1(\x)$ & $f_2(\x)$ & $f_6(\x)$\\
        $\tau(\x)$ & $f_4(\x)$ & $f_5(\x)$ & $f_6(\x)$ &$ f_7(\x)$ & $f_8(\x)$\\
        $\sigma$ & $1/2$ & $1$ & $1$ & $2$ & $4$\\
        \hline
    \end{tabular}
\end{table}

The defined scenarios are interesting because they represent different situations that we can face with real data. Indeed, scenario 1, although it seems simpler than the others (with a small noise level), is in fact a case that happens often, especially for marketing campaigns. In this scenario, by construction, there are no do-not-disturb clients. This results in an increasing monotonic Qini curve. In scenario 2, we introduce a group of do-not-disturb clients. In addition, we increase the noise level as well as the number of observations, but we reduce the number of variables. The average treatment effect is negative but a small group of persuadables is generated. In scenario 3, the main effect function is zero. Thus, the uplift is entirely guided by the treatment effect function. In scenario 4, we introduce a quadratic treatment effect function and scenario 5 is the most complex one. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/simulations/Qini_Curve_Scene_1.pdf}
    \includegraphics[width=0.49\textwidth]{figures/simulations/Qini_Curve_Scene_2.pdf}
    \includegraphics[width=0.49\textwidth]{figures/simulations/Qini_Curve_Scene_3.pdf}
    \includegraphics[width=0.49\textwidth]{figures/simulations/Qini_Curve_Scene_4.pdf}
    %\includegraphics[width=0.3\textwidth]{figures/simulations/Qini_Curve_Scene_5.pdf}
    \caption{Qini curves based on the ``true" uplift with respect to scenarios 1-4 of Table~\ref{tab:scenarios}.}
    \label{fig:qini_curves_scene}
\end{figure}


\paragraph{Benchmarks and implementation}
Each run of each simulation generates a dataset, which we split into training ($40\%$), validation ($30\%$), and test samples ($30\%$). We use the training and the validation sets to fit and fine-tune the models. Note that fine-tuning is specific to the type of the model, e.g. for a neural network, we fine-tune the learning rate and the regularization constant but for random forests, we fine-tune the number of trees as well as the depth of each tree. Then, we score the test samples with the fine-tuned models and compute performance metrics. We repeat each experiment $20$ times.

For each simulated dataset, we implement the following models:
\begin{enumerate}
    \item[(a)] a multivariate logistic regression, i.e. a twin model with no hidden layer that optimizes the Binomial likelihood. This is the baseline model, and we will refer to it as \textit{Logistic}. For fair comparison, we use the twin neural architecture and $L_1$ regularization.
    \item[(b)] our twin models, i.e. models (with and without hidden layers) that optimize the augmented loss function \eqref{eq:augmented_loss_function} to estimate the regression parameters. We denote these models by \textit{Twin$_{\mu}$} and \textit{Twin$_{\mathrm{NN}}$}.
    \item[(c)] a Qini-based uplift regression model that uses several LHS structures to search for the optimal parameters (see \citep{belba2019qbased} for more details). We denote this model by \textit{Qini-based}.
    \item[(d)] two types of random forests designed for causal inference (see \citep{athey2019generalized} for more details). This method uses honest estimation, i.e., it does not use the same information for the partition of the covariates space and for the estimation of the uplift. We denote these models by \textit{Causal Forest} and \textit{Causal Forest (Honest)} without and with honest estimation respectively.
    \item[(e)] two types of random forests designed for uplift (see \citep{rzepakowski2010decision,guelman2012random} for more details). This method uses different split criteria. We denote these models by \textit{Uplift Random Forest (KL)} and \textit{Uplift Random Forest (ED)} for Kullback-Leibler and Euclidean split criterion respectively.
\end{enumerate}



\paragraph{Results} All results are reported in Table~\ref{tab:all_scenarios}.

\begin{table}[!ht]
    \centering
    \begin{tabular}{l|c|ccccc}
        \hline
        Method & Hidden-Layer Size & 1 & 2 & 3 & 4 & 5 \\
        \hline
        {\it Logistic} && $0.75$ & $1.80$  & $3.50$ & $0.98$ & $2.59$\\
        {\it Qini-based} && $1.02$ & $\bf2.68$ & $4.36$ & $1.09$ & $2.94$\\
        {\it Twin$_{\mu}$} && $\bf1.24$  & $2.32$ & $\bf4.41$ & $\bf1.20$ & $\bf3.12$\\
        \hline
        {\it Twin$_{\mathrm{NN}}$}
        & $64$  & $1.54$  & $2.61$ & $\bf 4.91$ & $1.22$ & $3.10$ \\
        & $128$ & $1.56$  & $2.54$ & $4.80$ & $1.28$ & $3.16$\\
        & $201$ & $\bf 1.63$ & $\bf 2.67$  & $4.86$ & $1.30$ & $3.14$\\
        & $256$ & $1.57$ & $2.65$ & $4.78$ & $\bf 1.32$ & $3.26$ \\
        & $512$ & $1.60$ & $2.49$ & $4.64$ & $1.18$ & $\bf 3.35$\\
        \hline
        & $340/512$ & $1.67$  & $2.63$ & $5.03$ & $1.35$ & $3.58$\\
        \hline
        {\it Causal Forest} & &$0.75$ & $2.22$ & $4.42$ & $0.94$ & $2.79$ \\
        {\it Causal Forest (Honest)} && $0.75$  & $2.51$ & $4.53$ & $1.14$ & $3.07$\\
        {\it Uplift Random Forest (KL)} && $0.74$ & $2.52$ & $4.02$ & $1.01$& $2.19$ \\
        {\it Uplift Random Forest (ED)} && $0.68$ & $2.42$ & $4.18$ & $0.99$ & $2.33$ \\
        \hline
    \end{tabular}
    \vspace{2mm}
    \caption{Summary: models comparison in terms of $\qadj$.}
    \label{tab:all_scenarios}
\end{table}


\paragraph{The optimization criterion}

In this part of the analysis, we focus on the simple model (i.e. no hidden layer {\vahid [do you mean the logistic regression with interaction terms, better to refer with eqref to the right model to be precise]}), $\mu_{1t}(\x, \boldsymbol{\theta})$, defined in \eqref{eq:neural_network_1}. The goal is to compare three different ways to estimate the parameters. The {\it Logistic} method optimizes the penalized Binomial likelihood, as in the case of a {\it lasso} logistic regression. The {\it Qini-based} is a two-stage method which also makes use of the $L_1$ regularization. The methodology is based on $\qadj$ and imposing sparsity using the lasso. The $\qadj$ is a difficult statistic to compute, maximizing it directly is not an easy task. Therefore, the {\it Qini-based} first applies the pathwise coordinate descent algorithm \citep{friedman2007pathwise} to compute a sequence of critical regularization values and corresponding (sparse) model parameters. Then, it uses a derivative-free optimization algorithm (Latin Hypercube Sampling or LHS) to explore the parameters space in order to find the optimal model. The {\it Augmented loss} method optimizes our augmented loss function defined in \eqref{eq:augmented_loss_function} with $L_1$ regularization. Table~\ref{tab:param_estimation_results} shows the averaged results on the test dataset, for different scenarios. 

\begin{table}[!ht]
    \centering
    \caption{Comparison of parameter estimation for the $\mu_{1t}(\x, \boldsymbol{\theta})$ model in terms of $\qadj$.}
    \label{tab:param_estimation_results}
    \begin{tabular}{l|ccccc}
        Scenarios & 1 & 2 & 3 & 4 & 5\\
        Method & & & & & \\
        \hline
        {\it Logistic + $L_1$} & $0.75$ & $1.80$  & $3.50$ & $0.98$ & $2.59$\\
        {\it Qini-based} & $1.02$ & $\bf2.68$ & $4.36$ & $1.09$ & $2.94$\\
        {\it Augmented loss + $L_1$} & $\bf1.24$  & $2.32$ & $\bf4.41$ & $\bf1.20$ & $\bf3.12$\\
        \hline
    \end{tabular}
\end{table}


If we pick “winners” in each of the simulation scenarios based on which
method has the highest $\qadj$, {\it AL} would win all scenarios except for the second one. In scenario 2, the {\it Qini-based} model has the highest $\qadj$. In general both methods outperform the {\it Logistic} model.

\paragraph{Beyond linearity}

Ensemble methods are amongst the most powerful for the uplift case \citep{soltys2015ensemble}. A method that has proven to be very effective in estimating individual treatment effects is one based on generalized random forests \citep{athey2019generalized}. This method uses honest estimation, i.e., it does not use the same information for the partition of the covariates space and for the estimation of the uplift. This has the effect of reducing overfitting. Another candidate that we consider in our experiments is also based on random forests and designed for uplift \citep{rzepakowski2010decision,guelman2012random}. For this method, we consider two different split criteria, one based on the Kullback-Leibler divergence and one based on the Euclidean distance. In Table~\ref{tab:beyond_linearity_results}, we compare these methods to our neural-network version defined in \eqref{eq:neural_network_2}, that is, $\mathrm{NN}_{1t}(\x, \mathbf{W})$  with $m=2p+1$ hidden neurons. Here, we only consider $L_1$ regularization on the model's parameters.

\begin{table}[!ht]
    \centering
    \caption{{\vahid [bad table caption, why is it called AL? what is CF? URF? remember a table caption must be self contained.] Rethink about abbreviations, do not abbreviate if it is not necessary, otherwise it explodes your caption.}Comparison of non-linear models in terms of $\qadj$. The {\it AL} method optimizes the $\mathrm{NN}_{1t}(\x, \mathbf{W})$ model with $m=2p+1$ hidden neurons and $L_1$ regularization.}
    \label{tab:beyond_linearity_results}
    \begin{tabular}{l|ccccc}
        Scenarios & 1 & 2 & 3 & 4 & 5\\
        Method & & & & &\\
        \hline
        {\it AL$_{(p+1)\times m}$} & $\bf 1.63$ & $\bf 2.67$  & $\bf 4.86$ & $\bf 1.30$ & $\bf 3.14$\\
        {\it CF} & $0.75$ & $2.22$ & $4.42$ & $0.94$ & $2.79$ \\
        {\it CF$_{h}$} & $0.75$  & $2.51$ & $4.53$ & $1.14$ & $3.07$\\
        {\it URF$_{\mathrm{KL}}$} & $0.74$ & $2.52$ & $4.02$ & $1.01$& $2.19$ \\
        {\it URF$_{\mathrm{ED}}$} & $0.68$ & $2.42$ & $4.18$ & $0.99$ & $2.33$ \\
        \hline
    \end{tabular}
   
\end{table}



We observe that the random forests tend to overfit for several scenarios, with the exception of the honesty criteria which seems to mitigate this problem. On the other hand, we observe a good adequacy of the twin model in all scenarios. Overall, the results of {\it AL} appear to outperform all other methods significantly (based on  Wilcoxon signed-rank test \citep{wilcoxon1992individual}).

\paragraph{Parameter size}
{\vahid [this section is messy. simplify your paragraphs. I got lost.]}
Neural networks have two main hyper-parameters that control the architecture or topology of the network: the number of hidden layers and the number of nodes in each hidden layer. In the previous simulations, we fixed the number of hidden layers to $1$ and the number of nodes in the hidden layer to $2p+1$ as per Theorem~\ref{theorem}. However, the number of nodes can be seen as a hyper-parameter as well. 

Here, we vary the number of nodes to assess the impact on predictive performance, using either $m=64, 128, 256$ or $m=512$ nodes.  In Table~\ref{tab:hidden_neurons_results}, we report the averaged results. As we can see, there is not one optimal value of $m$ among the ones we compare that gives the best model for all scenarios. Depending on the scenario, we observe clear differences in terms of performance. 

For scenario 1, in which $p = 200$, we see that the best model is reached for $m = 512$; for scenario 2 and scenario 3, the model performs best with $m = 64$ and $m = 256$ respectively, and finally with $m = 256$ and $m = 512$ for scenarios 4 and 5. Therefore, in practice, for a specific dataset, it is important to consider the number of neurons in the hidden layer as a hyper-parameter that can be fine-tuned by cross-validation.

\begin{table}[!ht]
    \centering
    \caption{Fine-tuning the number of nodes in terms of $\qadj$. The {\it AL} method optimizes the $\mathrm{NN}_{1t}(\x, \mathbf{W})$ model with $m$ hidden neurons and $L_1$ regularization.}
    \label{tab:hidden_neurons_results}
    \begin{tabular}{l|l|ccccc}
        Scenarios &$m$ & 1 & 2 & 3 & 4 & 5\\
        Method &&&&&&\\
        \hline
        {\it AL$_{(p+1)\times m}$} 
        & $64$ & $1.54$  & $2.61$ & $\bf 4.91$ & $1.22$ & $3.10$ \\
        & $128$ & $1.56$  & $2.54$ & $4.80$ & $1.28$ & $3.16$\\
        & $256$ & $1.57$ & $\bf 2.65$ & $4.78$ & $\bf 1.32$ & $3.26$ \\
        & $512$ & $\bf 1.60$ & $2.49$ & $4.64$ & $1.18$ & $\bf 3.35$\\
               \hline
    \end{tabular}
\end{table}

Choosing the number of hidden neurons by cross-validation is very common in practice. This is part of architecture search. However, choosing among a few values does not necessarily mean that all the selected model's neurons are useful. As discussed in Section~\ref{sec:choice_reg_function}, the use of the group lasso penalization on the weight matrix allows to automatically fine-tune the number of hidden neurons (i.e. pruning). This has the effect of increasing the performance of the underlying models from a predictive point of view, as shown in Table~\ref{tab:hidden_neurons_pruning}. Thus, we suggest to start with a fairly large number of hidden neurons (e.g. $m \geq 2p +1$), and to let the optimization determine the number of active neurons needed for a specific dataset.

\begin{table}[!ht]
    \centering
    \caption{Performance when automatically pruning the number of nodes. The {\it AL} method optimizes the $\mathrm{NN}_{1t}(\x, \mathbf{W})$ model with $m=512$ hidden neurons and $L_1$ + \emph{group lasso} regularization functions.}
    \label{tab:hidden_neurons_pruning}
    \begin{tabular}{l|l|ccccc}
        Scenarios & & 1 & 2 & 3 & 4 & 5\\
        \hline
        {\it AL$_{(p+1)\times 512}$} 
        & $\hat{m}$ & $422$  & $97$ & $48$ & $178$ & $340$ \\
        & $\qadj$ & $1.67$  & $2.63$ & $5.03$ & $1.35$ & $3.58$\\
        \hline
    \end{tabular}
\end{table}


\paragraph{Summary} The number of hidden layers can also be seen as a hyper-parameter for the neural network architecture. In our experiments, increasing the number of hidden layers did not improve the performance significantly. When we fix the initial number of hidden neurons to $p+1$ and $p$ for the $2$ hidden layer, in scenarios 1 and 5, the average $\qadj$ are $1.59$ and $3.39$ respectively.  We report the averaged results as well as a summary of all previous experiments in Table~\ref{tab:hidden_layers_results}. For random forests uplift models, we report the best score between the four used methods. For scenarios 1, 3, 4 and 5, the best results are obtained with the $1$-hidden layer twin model. For scenario 2, the {\it Qini-based} uplift regression achieves the highest $\qadj$, tying with the $1$-hidden layer twin model (i.e. $2.68$ vs. $2.67$).
{\vahid[This is not summary. The conclusion is what? Scnarios change the performance? number of hidden units are not important? lasso and group lasso finds the moinimal $m$? ]}
\begin{table}[H]
    \centering
    \caption{Summary: performance of fitted models in terms of $\qadj$.}
    \label{tab:hidden_layers_results}
    \begin{tabular}{l|l|ccccc}
        Scenarios &$h$ & 1 & 2 & 3 & 4 & 5\\
        Method &&&&&&\\
        \hline
        {\it AL + $L_1$} & $0$ & $1.24$  & $2.32$ & $4.41$ & $1.20$ & $3.12$\\
        {\it Logistic + $L_1$} & - & $0.75$ & $1.80$  & $3.50$ & $0.98$ & $2.59$\\
        {\it Qini-based} & - & $1.02$ & $\bf 2.68$ & $4.36$ & $1.09$ & $2.94$\\
        \hline
        {\it AL + $L_1$} & $1$ & $1.63$ & $2.67$  & $4.91$ & $1.32$ & $3.35$\\
        {\it AL + $L_1$ + \emph{group lasso}} & $1$ & $\bf 1.67$  & $2.63$ & $\bf5.03$ & $\bf1.35$ & $\bf3.58$\\
        %  & $2$ & $1.59$ & $2.36$ & $4.92$ & $1.38$ & $ 3.39$ \\
        Best {\it RF} & - & $0.75$ & $2.52$ & $4.53$ & $ 1.14$ & $3.07$\\
        \hline
    \end{tabular}
\end{table}


==> others/foothill.tex <==
\subsection{Alternative losses and activations}

The choice of loss functions and activations in deep networks has a significant effect on the training dynamics and task performance.

\subsubsection{Definitions}

Foothill function \citep{belbahri2019foothill} is defined as

\begin{align}
    p_{\alpha,\beta}(x) = \alpha x~ \mathrm{tanh}\left( \frac{\beta x}{2} \right).
    \label{eq:reswish}
\end{align}

where $\mathrm{tanh}(.)$ is the hyperbolic tangent function, $\alpha > 0$ is a shape parameter and $\beta > 0$ is a scale parameter. % and $\mu$ a location parameter. 
The function is symmetric about $0$ (see Figure \ref{fig:foothill}, left panel). The first and the second derivatives (see Figure \ref{fig:foothill}, right panel) of foothill are 

\begin{align*}
    \frac{dp_{\alpha,\beta}(x)}{dx} = \alpha ~ \mathrm{tanh}\left( \frac{\beta x}{2} \right) + \frac{1}{2} \alpha \beta x ~ \mathrm{sech}^2\left( \frac{\beta x}{2} \right), \\
     \frac{d^2p_{\alpha,\beta}(x)}{d^2x} = \frac{1}{2} \alpha \beta~ \mathrm{sech}^2\left( \frac{\beta x}{2} \right) \left\{  2 - \beta x ~ \mathrm{tanh}\left( \frac{\beta x}{2} \right) \right\},
\end{align*}
where $\mathrm{sech}(.)$ is the hyperbolic secant function.

\begin{figure}[htb]
    \centering
    \begin{tikzpicture}[scale=0.5]
    \begin{axis}[
      axis x line=middle, axis y line=middle, samples = 200,
      ylabel={$p_{\alpha,\beta}(x)$},ylabel style={font=\Large, yshift=3pt},
      ymin=-0.1, ymax=2.5, ytick={0,1,2},
      xmin=-3, xmax=3, xtick={-1, 0, 1}
    ]
    \addplot[black, domain=-2.4:2.4, dashed]{1*2*(x-0)*((1+pow(e,-1*(x-0)))^(-1) - 0.5)};
    \addplot[black, domain=-2:2, smooth]{1*2*(x-0)*((1+pow(e,-50*(x-0)))^(-1) - 0.5)};
    \end{axis}
    \end{tikzpicture} 
    \hspace{0.5cm}% NO SPACE!
    \begin{tikzpicture}[scale=0.5]
            \begin{axis}[
      axis x line=middle, axis y line=middle, samples = 100,  ylabel={$\frac{d^{(l)}p_{1,1}(x)}{d^{(l)}x}$},ylabel style={font=\Large, yshift=3pt}, ymin=-2, ymax=2, ytick={-1,0,1}, xtick={-2.4, -1, 0, 1, 2.4},
      xmin=-4, xmax=4
    ]
    \addplot[black, domain=-4:4, dashed]{2*(1+pow(e,-1*x))^(-1)*(1+1*x*pow(e,-1*x)*(1+pow(e,-1*x))^(-1)))-1};
    \addplot[black, domain=-4:4, smooth]{2 * (-1^2 * x * pow(e, -1*x) * (1+pow(e,-1*x))^(-2) + 2 * 1^2 * x * pow(e, -2*1*x) * (1+pow(e,-1*x))^(-3) + 2 * 1 * pow(e, -1*x) * (1+pow(e,-1*x))^(-2)) };
    \end{axis}
    \end{tikzpicture} 
    \caption{Left panel: Regularization function \eqref{eq:reswish} for $\alpha=1$, $\beta=1$ (solid line)  and $\alpha=1$, $\beta = 50$ (dashed line). Right panel: The first (dashed line) and the second (solid line) derivatives of the regularization function \eqref{eq:reswish} for $\alpha=1$ and $\beta=1$.
    }
    \label{fig:foothill}
\end{figure}

\subsubsection{Properties}

The regularization function (\ref{eq:reswish}) has several interesting properties. It is infinitely differentiable and symmetric about the origin, $$ p_{\alpha,\beta}(x) =  p_{\alpha,\beta}(-x).$$ 
Also, it is flexible enough to approximate the lasso \cite{Tibshirani_lasso_1996} and Ridge penalties \cite{hoerl1970ridge} for particular values of $\alpha$ and $\beta$. The following properties suggest that this function could be considered as a quasiconvex alternative to the elastic net penalty \cite{zou2005regularization}.

\begin{property}  For $\alpha=1$ and $\beta \rightarrow \infty$, the foothill penalty (\ref{eq:reswish}) converges to the lasso penalty.
\end{property}

\emph{Proof.} For $x>0$, it is easy to see that
\begin{flalign*}
    \lim_{\beta \rightarrow +\infty}& \mathrm{tanh}\left( \frac{\beta x}{2} \right) = 1,\\
	\lim_{\beta \rightarrow +\infty}& p_{\alpha, \beta}(x) = x.
\end{flalign*}

Equivalently, for negative $x$, as $p_{\alpha, \beta}(x)$ is symmetric about the origin, then $\lim_{\beta \rightarrow +\infty} p_{\alpha, \beta}(x) = -x$, which is equivalent to $p_{\alpha, \beta}(x) \rightarrow |x|$ when $\beta \rightarrow +\infty$.

\begin{property}  For $\alpha>0$, $\beta>0$, and $\beta = 2 / \alpha$ the foothill penalty  (\ref{eq:reswish}) approximates the Ridge penalty in a given interval $[-c ; c]$.
\end{property}

\emph{Proof.} Let us study this property formally. Take the Taylor expansion of (\ref{eq:reswish}), 
\begin{align}
    p_{\alpha, \beta}(x) \approx \frac{\alpha\beta}{2} x^2 - \frac{\alpha\beta^3}{24} x^4 + \frac{\alpha\beta^5}{240} x^6 + \mathrm{O}(x^8).
	\label{eq:taylor}
\end{align}

And, for a given $c>0$, 
\begin{align}
    \int_{0}^{c} \left( \frac{\alpha\beta}{2} x^2 - p_{\alpha, \beta}(x)  \right)^2 dx \approx \frac{\alpha^2\beta^6}{5184} c^9 + \mathrm{O}(c^{11}).
	\label{eq:approxridge}
\end{align}

The integral in (\ref{eq:approxridge}) diverges if $c$ tends to infinity, but for a finite positive number $c$, one can numerically estimate the minimal distance between the $L_2$ norm and (\ref{eq:reswish}) with a tiny approximation error. This can be achieved by taking $\beta = 2 / \alpha$ and (\ref{eq:approxridge}) becomes 
\begin{align}
    \int_{0}^{c} \left( x^2 - p_{\alpha, \beta}(x)  \right)^2 dx \approx \frac{1}{81\alpha^4} c^9 + \mathrm{O}(c^{11}) = \varepsilon_c .
	\label{eq:approxridge2}
\end{align}
For large values of $\alpha$, the error $\varepsilon_c$ is negligible, see for example Figure \ref{fig:approxridge} where the regularization function (\ref{eq:reswish}) approximates the Ridge penalty almost perfectly within $[-5 ; 5]$. Furthermore, for fixed parameters, note that 
\begin{align*}
    \lim_{x \rightarrow +\infty} p_{\alpha, \beta}(x) - \alpha x = 0, ~~\mathrm{and}~~  
	\lim_{x \rightarrow -\infty} p_{\alpha, \beta}(x) + \alpha x = 0.
\end{align*}

Hence it is also interesting to note that (\ref{eq:reswish}) behaves like a polynomial function for small values of $x$, and like a linear function for large values. Therefore, using it as a loss function (instead of a regularization), (\ref{eq:reswish}) behaves like the Huber loss used in practice for robust estimation \cite{huber1964robust}. Figure \ref{fig:approxridge} shows that (\ref{eq:reswish}) is bounded between the Huber loss and the squared error loss.

\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.4]{figures/fig/huber_like_foothill.pdf} 
    \caption{Plots of the Ridge, the foothill penalty with $\alpha = 16$ and $\beta=0.125$ and twice the Huber loss. The solid blue line represents the foothill penalty, the dashed line represents the Ridge one (upper bound) and Huber (lower bound) is represented in dotted line.}
    \label{fig:approxridge}
\end{figure}

\begin{property}  Saddle points of $p_{\alpha, \beta}(x)$ are $x_0 \approx \pm 2.3994/\beta$ and $p_{\alpha, \beta}(x_0) = \frac{2 \alpha }{\beta}$.
\end{property}

\emph{Proof.} Indeed, the second order derivative vanishes at
\begin{align*}
     2 - \beta x ~ \mathrm{tanh}\left( \frac{\beta x}{2} \right) = 0,\\
\end{align*}
which is solved by an iterative method for  $\beta x \approx \pm 2.3994$. This implies
\begin{align*}
     \beta x_0 ~ \mathrm{tanh}\left( \frac{\beta x_0}{2} \right) = 2,
\end{align*}
or equivalently
\begin{align*}
	p_{\alpha, \beta}(x_0) = \frac{2 \alpha }{\beta}.
\end{align*}

\begin{property}  The function $p_{\alpha, \beta}(x)$ is quasiconvex.
\end{property}

\emph{Proof.} It is straight forward to show that $p_{\alpha, \beta}(x)$ is decreasing from $-\infty$ to $0$ and increasing from $0$ to $+\infty$ and any monotonic function is quasiconvex (see Figure \ref{fig:foothill}, right panel).



\vspace{0.5cm}
Table \ref{tab:relation} suggests that foothill has the flexibility to be used for feature selection regularizer such as the lasso or used only to shrink the estimator in order to prevent over-fitting like the Ridge. Finally, it also can be used as a loss function for robust regression as an alternative to the Huber loss.

\begin{table}[htb]
\caption{Relationship to other functions} \label{tab:relation}
\begin{center}
\begin{tabular}{l@{\hspace{0.1in}}l@{\hspace{0.1in}}l@{\hspace{0.1in}}l}
  & Shape $\alpha$ & Scale $\beta$ & Function\\
\hline
Lasso        & $1$ & $+\infty$  & $p_{\alpha, \beta}(x)=|x|$\\
Ridge        & $+\infty$ & $2 / \alpha$ & $p_{\alpha, \beta}(x)=x^2$\\
Huber & $< +\infty$ & $2 / \alpha$ &  $p_{\alpha,\beta}(x) = \alpha x~ \mathrm{tanh}\left( \frac{x}{\alpha} \right)$\\
Foothill   & $1$ & $2$ & $p_{\alpha, \beta}(x)=x \mathrm{tanh}(x)$\\
\end{tabular}
\end{center}
\end{table}


==> others/litterature.tex <==
We give a brief summary of some of the conceptual steps that led to today's mathematical understanding of the universal approximation theorems. For a thorough and extensive historical bibliography on neural networks, \cite{schmidhuber2015deep} compiled 888 references. See \cite{goodfellow2016deep} for an elementary well documented introduction to the subject.

\section{Universal approximation theorems}

A neural network (NN; for a definition, see e.g. \cite{pinkus1999approximation} or \cite{calin2020deep}) transforms an input $x\in D\subset\mathbb{R}^{n}$ into an output $\widetilde{y}=\Phi\left(  x\right)  \in\mathbb{R}$. As such it is a concrete real function of $n$ real variables, $n$ being a priori an arbitrary positive integer. A natural question that has been asked for a long time is the following: can this NN (with an appropriate architecture) approximate functions of a given class (common example: multivariate continuous functions defined on $D=K$, a compact subset of $\mathbb{R}^{n}$, but more general function spaces, such as $L^{p}$ spaces, are usually the proper framework from an abstract mathematical viewpoint) \citep{mhaskar1996system}? In other words, can a NN generate a topologically dense subset of the function class in question? For example, in the case of a normed vector space, given $\epsilon>0$, is there and, if so, can one actually construct at a reasonable cost a NN such that

\[
\left\Vert f-\widetilde{y}\right\Vert <\epsilon\text{ ?}%
\]

A related question (among many other researchers are addressing \citep{fan2020universal}) is: to what extent does the choice of the norm (topology) affect this existence and/or construction?

The proper mathematical interpretation of NN is based on the universal
approximation theorems (UAT). The UAT are roughly divided into two categories:

\begin{enumerate}
\item arbitrary number of neurons in the case of {\it shallow} neural networks (SNN, arbitrary width). This is the classical case. It goes back to the pioneering work of the 1940-1980's;

\item arbitrary number of layers with {\it deep} neural networks (DNN, arbitrary
depth). In practice, the latter have proven to be more efficient
\citep{mhaskar2019function}. It is always possible to build a SNN to emulate a DNN. However the number of neurons grows exponentially in order to obtain a
comparable performance (in terms of error) \citep{telgarsky2016benefits,eldan2016power}.
\end{enumerate}

In this sense, the UAT are representations of classical existence theorems. They implement the construction (i.e. find the appropriate weights) of the approximation of large classes of functions \citep{paluzo2020two}. However, they do not say how one explicitly (with a formula or an algorithm) finds this approximation (weights).

We give a brief summary of some of the conceptual steps that led to today's mathematical understanding of the UAT.

\begin{itemize}
\item The Kolmogorov--Arnold representation (or superposition) theorem \citep{kolmogorov1957representation} states that any continuous real multivariate function can be represented by a superposition of real one-variable continuous functions $f:\mathbb{R}^{n}\rightarrow\mathbb{R}$:
\[
f(x)  =\sum_{i=0}^{2n}\Phi_{i}\left(  \sum_{j=1}^{n}\phi
_{i,j}(x_{j})  \right)
\]
This theorem gives a partial answer to Hilbert's 13th problem \citep{akashi2001application,khesin2014arnold}. A construction is proposed by \cite{polar2020urysohn}.

\item Prior to the 1980s \citep{mcculloch1943logical,fukushima1975cognitron}, NN architectures were shallow. An understanding of SNN gives a good appreciation of DNN.

\item The Kolmogorov-Arnold theorem gives an exact representation of the function $f(x)$. This representation proves to be very complex (fractal nature) and computationally very slow, therefore unusable in NN. The accuracy condition had to be relaxed for an approximation condition ($L^{p}$
or uniform norm). The optimal solution is sought by iterative methods (the
gradient descent, introduced by Jacques Hadamard in 1908, being the most
popular). Pioneering modern work is due to \cite{cybenko1989approximation} for
sigmoid activation functions (arbitrary width), \cite{funahashi1989approximate}, \cite{hornik1991approximation} (he showed that UAT was
potentially constructible using a multilayer architecture of the NN rather
than a specific choice of the activation function), \cite{barron1993universal} (bounds on smooth function errors), etc...

\item  \cite{leshno1993multilayer} and \cite{pinkus1999approximation} have
shown that the universal approximation property (see \cite{kratsios2019universal} for a
definition) is equivalent to a non polynomial activation function.
\end{itemize}

\begin{theorem}
(\cite{cybenko1989approximation,hornik1991approximation,pinkus1999approximation}). Let $n\in\mathbb{N}$, $K\subset\mathbb{R}^{n}$ compact, $f:K\rightarrow\mathbb{R}$ continuous, $\rho:\mathbb{R}\rightarrow\mathbb{R}$ non polynomial and continuous, and let $\epsilon>0$. Then there exists a
two-layer NN $\Phi$ with activation function $\rho$ such that
\[
\left\Vert \Phi-f\right\Vert _{\infty}<\epsilon.
\]
\end{theorem}

We also note that DNN have demonstrated their capabilities in the approximation of functions \citep{liang2016deep,yarotsky2017error,fan2020universal}. They are found to have good experimental (empirical) performance, but it is largely unknown why. This is a very active area of research \cite{caterini2018deep}.

\begin{theorem}
(\cite{lu2017expressive}) Let  $f:\mathbb{R}^{n}\rightarrow\mathbb{R}$ be Lebesgue-integrable and $\epsilon>0$. Then there exists a ReLU
network of width $\leq n+4$ such that
\[
\int_{\mathbb{R}^{n}}\left\vert \Phi\left(  x\right)  -f\left(  x\right)  \right\vert dx<\epsilon
\]

\end{theorem}

\begin{definition}
(\cite{kidger2020universal}) Let $\rho:\mathbb{R}\rightarrow\mathbb{R}$ and $n,m,k\in\mathbb{N}$. Then let $NN_{n,m,k}$ represent the class of functions $\mathbb{R}^{n}\rightarrow\mathbb{R}^{m}$ described by feedforward neural networks with $n$ neurons in the input layer, $m$ neurons in the output layer, and an arbitrary number of hidden layers, each with $k$ neurons with activation function $\rho$. Every neuron in the output layer has the identity activation function.
\end{definition}

\begin{theorem}
(\cite{kidger2020universal}) Let $\rho:\mathbb{R}\rightarrow\mathbb{R}$ be any non-affine continuous function which is continuously differentiable at
at least one point, with non-zero derivative at that point. Let $K\subset\mathbb{R}^{n}$ be compact. Then NN$_{n,m,n+m+2}$ is dense in $C\left(  K,\mathbb{R}^{m}\right)$ with respect to the uniform norm.
\end{theorem}


\section{Low-rank approximation}

Due to its fundamental role in Machine Learning, a huge literature is devoted
to the singular value decomposition (SVD) of a matrix. We refer to some of the
well respected texts: \cite{strang1993introduction}, \cite{trefethen1997numerical}, \cite{watkins2004fundamentals}, \cite{gentle2007matrix}, \cite{elden2007matrix}, \cite{lange2010numerical},
and \cite{yanai2011projection} for
instance. Let $A\in \mathbb{R}^{m\times n}$ be a matrix of rank $r$. Its SVD consists in factoring $A$ as
\[
A=U\Sigma V^\top=\sum_{i=1}^{r}\sigma_{i}\u_{i}\v_{i}^\top
\]
where $U\in\mathbb{R}^{m\times m}$ and $V\in\mathbb{R}^{n\times n}$ are orthogonal square matrices, and $\Sigma\in\mathbb{R}^{m\times n}$ (\textquotedblleft diagonal\textquotedblright\ rectangular matrix of the ordered singular values: $\sigma_{1}\geq\ldots\geq\sigma _{r}>\sigma_{r+1}=\ldots=0=\sigma_{\min\{m,n\}}$). This
decomposition, and the related principal component analysis (PCA), has several
uses in Data Analysis. Written as $AV=U\Sigma$, SVD says that there exist orthogonal matrices $U$ and $V$ such that $A$ maps the columns $\v_{i}$ of $V$ (right singular vectors of $A$, directions or principal axes in the PCA parlance) into the columns $\u_{i}$ of $U$ (left singular vectors of $A$) such as
\[
A\v_{i}=\sigma_{i}\u_{i},
\]
the principal components.

Given a positive integer $1\leq k\leq r$, introduce the truncated matrices
$U_{k}=\left[  \u_{1},\ldots,\u_{k}\right]  \in \mathbb{R}^{m\times k}$, $V_{k}=\left[  \v_{1},\ldots,\v_{k}\right]  \in \mathbb{R}^{k\times n}$, and $\Sigma_{k}=\mathrm{diag}(  \sigma_{1},\ldots,\sigma_{k}) \in \mathbb{R}^{k\times k}$. Then the matrix of rank $k$
\[
A_{k}=U_{k}\Sigma_{k}V_{k}^\top=\sum_{i=1}^{k}\sigma_{i}\u_{i}\v_{i}^\top
\]
is an optimal lower-rank approximation of $A$ in the sense of both the
Frobenius norm and the $L_2$-norm. Indeed, the Eckart--Young--Mirsky theorem (for
a proof, see \cite{markovsky2012low}) states that among all matrices $B\in\mathbb{R}^{m\times n}$ of a given rank $k\leq r$, the one closest to $A$ is
$\hat{A}=A_{k}$, i.e.

\begin{align*}
\inf_{\mathrm{rank}(B)=k}\left\Vert A-B\right\Vert _{F} &  =\left\Vert
A-\hat{A}\right\Vert _{F}=\sqrt{\sum_{i=k+1}^{r}\sigma_{i}^{2}},\\
\inf_{\mathrm{rank}(B)=k}\left\Vert A-B\right\Vert _{2} &  =\left\Vert
A-\hat{A}\right\Vert _{2}=\sigma_{k+1}.
\end{align*}

Furthermore, the approximating matrix $\hat{A}$ is unique if and only if
$\sigma_{k+1}\neq\sigma_{k}$ \citep{markovsky2012low}. The theorem was proved in 1907 by Schmidt (of the Gram-Schmidt procedure) for the Frobenius norm \citep{leon2013gram}. A constructive solution was given by \cite{eckart1936approximation}. This solution was
shown by \cite{mirsky1960symmetric} to hold for all unitarily invariant norms. A further generalization addressing collinearity issues was proposed by \cite{golub1987generalization}. See \cite{stewart1993early} for historical details. 

One interpretation of the decomposition $A_{k}=U_{k}\Sigma_{k}V_{k}^{T}$ is as
a compression/learning linear procedure of the data matrix $A$ (in other
words, a dimension reduction method). Indeed, since the SVD extracts data in
the direction with the highest variance (and going down to those with the
lowest variance), matrix $U_{k}$ is the compression matrix in the first $k$
directions, matrix $\Sigma_{k}$ contains the amount of error (cost function)
we tolerate, and $V_{k}$ is the decompression matrix. If we keep all the non
zero singular values ($k=r$), there is theoretically no loss in the
compression (assuming that the data in $A$ are exact). If we drop the small
singular values (set them to $0$), it is not possible to reconstruct the
initial matrix $A$ exactly, but we obtain a matrix $A_{k}$ that is close. In
other words, the SVD decomposition is a way to control the loss of information
from $A$ under a predetermined level.

The assumption (routinely validated in image processing, for example) in the
above approach is that the components (columns of $U$) of the small singular
values contain little information (mostly \textquotedblleft
noise\textquotedblright) and should be discarded. However, the low-rank matrix approximation is easily seen not to be optimal if used to solve the linear regression problem (hence as a predictive tool) $y=A\beta+\epsilon$, that is to minimize
\begin{equation}
    \inf_{\mathrm{rank}(B)=k}\left\Vert \y-B\bbeta\right\Vert . 
    \label{eq:svd_regression}
\end{equation}

While the SVD picks the parameter $k-$vector $\bbeta$ of minimum norm
\citep{elden2007matrix,lange2010numerical},

\begin{equation}
    \hat{\bbeta}=A_{k}^{\dag} \y=\sum_{i=1}^{k}\frac{1}{\sigma_{i}} \u_{i}^\top \y \v_{i},
    \label{eq:svd_reg_solution}
\end{equation}

where $A_{k}^{\dag}$ is the pseudoinverse of $A_{k}$, the general solution of
\eqref{eq:svd_regression} is unknown \citep{xiang2012optimal}. See also \cite{talwalkar2010matrix} for a discussion in the Machine Learning context.

Some authors \citep{jolliffe1982note,hadi1998some} warned against the misconceived (mainly due to collinearity considerations) use of \eqref{eq:svd_reg_solution} in an ordinary linear regression setting. Dropping some of the small singular values may result in ignoring significant variables, mainly because the approximation does not take into account the response variable $\y$. A partial solution is provided by the ridge regression \citep{hoerl1970ridge}. However, still from a predictive viewpoint, SVD may prove to be an interesting approach in deep neural networks \citep{bermeitinger2019singular}. Used for initialization in the first layer, SVD gave promising experimental results. Theoretical issues still need to be addressed.

\newpage

==> others/low_rank_smite.tex <==
\subsection{Low-rank and SMITE}

\textit{Comment from Alejandro Murua: We do not necessarily study low rank approximations of the matrix of weights. For this you will need indeed to get bounds on the distance between the estimated function and the approximation function. In Statistics, usually we just measure the statistical difference between two models (and not the distance between the two models). So instead of thinking of a reduced approximation of the weight matrix, we might just think of a model with a lower-rank matrix of weights. This in general will lead to a non-parametric estimator with lower variance and hopefully, only slightly increased bias. In this setup, methods to measure the statistical difference between the full model and the reduced model should be applied for each dataset. This is in contrast to the general approximation theory, where bounds on the approximation error over all possible datasets need to be found.}


We are interested in determining how complex the network ought to be to theoretically guarantee that the network would approximate an unknown target function $f$ up to a given accuracy $\epsilon > 0$. To measure the accuracy, we need a norm $\norm{\cdot}$ on some normed linear space. We work with $L_2$ norm.

We focus on a feed-forward neural network with one fully-connected hidden layer. Here the input layer (with $n$ neurons) and the hidden layer (with $m$ neurons) are assumed to be fully connected with a weight matrix $\mathbf W \in \real^{n \times m}$ with rank at most $p \leq \mathrm{min}(n,m)$. The domain for the input vector $\x$ is the $n$-dimensional hypercube $I^n = [0, 1]^n$, and the output layer only contains one neuron. The neural network can be expressed as 

$$\hat y = \hat f(\x\mid \mathbf  W) = \sum_{j=1}^m \alpha_j h(\mathbf w_j^\top\x + \beta_j) = \boldsymbol{\alpha} h(\x \mathbf{W} + \boldsymbol{\beta}).$$ 

Here $h(\cdot)$ is the activation function, $\mathbf w_j \in \real^n$ denotes the $j$-th column of the weight matrix $\mathbf W$, and $\alpha_j, \beta_j \in \real$ for $j = 1, \ldots, m$. Suppose $p$ is the rank of the matrix $\mathbf W$. We can denote it $\mathbf W_p$ and define the following trained model

$$\hat y_p = \boldsymbol{\alpha} h(\x \mathbf{W_p} + \boldsymbol{\beta}).$$ 


Let $r < p$ be an integer and define 

$$\hat y_r = \boldsymbol{\alpha} h(\x \mathbf{\hat W_r} + \boldsymbol{\beta}),$$

be the prediction from the model where $\mathbf{W_p}$ has been approximated with $\mathbf{\hat W_r}$ of rank $r$, that is, $\mathbf{\hat W_r} = \mathbf{\hat U \hat \Sigma_r \hat V^{\top}}$ where $\mathbf{\hat{U}, \hat{\Sigma_r}, \hat{V}\t} \in \real^{n\times r}, \real^{r\times r}, \real^{r \times m}$. This approximates the original weights $\mathbf W_p$ into reconstructed approximated weights $\mathbf{\hat{W_r}}$. 

The truncation process always keeps the first $r$ rows of $\mathbf U$ and columns of $\mathbf V\t$. The number of non-zero parameters in the truncated SVD is $r( n + m + 1)$. The compression ratio is the ratio between parameters after and before the decomposition which is calculated as $r( n + m + 1)/( nm )$. In addition, the weight matrix does not need to be reconstructed during inference where the input $\x$ can be directly multiplied with $\mathbf{\hat{U}, \hat{\Sigma_r}, \hat{V}\t}$ matrices, which takes lesser computation than direct multiplication of $\hat{\mathbf W_r}$ and $\x$. Therefore, we have the following development

\begin{align*}
\norm{ \hat y_p - \hat y_r }_2 &= \norm{\boldsymbol{\alpha} h(\x \mathbf{W_p} + \boldsymbol{\beta}) - \boldsymbol{\alpha} h(\x \mathbf{\hat W_r} + \boldsymbol{\beta})}_2  \\
&\leq \norm{\boldsymbol{\alpha}}_2 \norm{h(\x \mathbf{W_p} + \boldsymbol{\beta}) - h(\x \mathbf{\hat W_r} + \boldsymbol{\beta})}_2\\
&\leq \norm{\boldsymbol{\alpha}}_2 \norm{\x \mathbf{W_p} - \x \mathbf{\hat W_r}}_2 ~ \text{because $h(\cdot)$ is $1$-Lipschitz continuous}\\
&\leq \norm{\boldsymbol{\alpha}}_2 \norm{\x}_2 \norm{\mathbf{W_p} - \mathbf{\hat W_r}}_2\\
&\leq \norm{\boldsymbol{\alpha}}_2 \norm{\x}_2 \sigma_{r+1} ~ \text{by Eckart-Young Theorem \citep{eckart1936approximation}}\\
&\leq \Big( \sum_{j=1}^m \alpha_j ^ 2 \Big)^{1/2}  \sqrt{n} \sigma_{r+1}
\end{align*}

where $\sigma_{r+1}$ is the $(r+1)$th singular value of $\mathbf{W_p}$.





%\begin{table}[!ht]
%    \centering
%    \caption{Comparison of models complexity (TO, IE). The metric used is the adjusted Qini coefficient.}
%    \label{tab:low_rank_results}
%    \begin{tabular}{l|l|ccccc}
%        Scenarios &$m$ & 1 & 2 & 3 & 4 & 5\\
%        \hline
%        {\it TO$_{\hat\alpha,(p+1)\times m + m\times(2p+1)}$} & $1$ &  &  & & & $\bf 3.21$\\
%        & $2$ &  &  & & & $3.07$\\
%        & $8$ &  &  & & & $3.05$\\
%        & $16$ &  &  & & & $3.00$\\
%        & $32$ &  &  & & & $3.03$\\
%        & $64$ &  &  & & & $2.99$\\
%        \hline
%        {\it IE$_{(p+1)\times m  + m\times(2p+1)}$} & $1$ &  &  & & &  $3.14$\\
%        & $2$ &  &  & & &  $\bf 3.15$\\
%        & $8$ &  &  & & &  $\bf 3.15$\\
%        & $16$ &  &  & & &  $3.04$\\
%        & $32$ &  &  & & &  $3.03$\\
%        & $64$ &  &  & & &  $3.09$\\
%               \hline
%    \end{tabular}
%\end{table}



==> others/rf_ie_loss.tex <==

\newpage
\subsection*{Random Forests and IE loss}

\begin{table}[H]
    \centering
    \begin{tabular}{lrrrrrrrrrr}
    \toprule
    max\_depth &      1  &      2  &      3  &      4  &      5  &      6  &      7  &      8  &      9  &      10 \\
    n\_estimators &         &         &         &         &         &         &         &         &         &         \\
    \midrule
    10           &  0.0000 &  0.0000 &  0.4627 &  0.0000 &  0.0000 &  0.0847 &  0.6873 &  0.1620 &  0.6227 &  0.8690 \\
    60           &  0.0000 &  0.6076 &  0.2521 &  0.3716 &  0.7808 &  0.6221 &  0.9801 &  0.4200 &  \textcolor{blue}{0.6480} &  0.6447 \\
    110          &  0.2358 &  0.2152 &  0.4802 &  0.2579 &  0.6272 &  0.5698 &  0.7611 &  0.8179 &  0.9595 &  0.6621 \\
    160          &  0.7447 &  0.1843 &  0.2604 &  0.1395 &  0.6537 &  0.7644 &  0.7623 &  0.8682 &  0.6104 &  0.5373 \\
    210          &  0.6333 &  0.1896 &  0.3153 &  0.3784 &  0.5498 &  0.9748 &  0.5699 &  0.8745 &  \bf 1.1953 &  0.6199 \\
    \bottomrule
    \end{tabular}
    \caption{$\qadj$}
    \label{tab:my_label}
\end{table}

\begin{table}[H]
    \centering
    \begin{tabular}{lrrrrrrrrrr}
    \toprule
    max\_depth &       1  &       2  &       3  &       4  &       5  &       6  &       7  &       8  &       9  &       10 \\
    n\_estimators &          &          &          &          &          &          &          &          &          &          \\
    \midrule
    10           &  0.91698 &  0.89777 &  0.87211 &  0.88674 &  0.87344 &  0.86945 &  0.86670 &  0.86730 &  0.86579 &  0.86359 \\
    60           &  0.91405 &  0.89896 &  0.88380 &  0.88023 &  0.87313 &  0.86804 &  0.86168 &  0.86205 &  \bf 0.85797 &  0.85802 \\
    110          &  0.91569 &  0.89789 &  0.88678 &  0.88219 &  0.87444 &  0.87028 &  0.86275 &  0.86258 &  0.86004 &  0.86072 \\
    160          &  0.91891 &  0.89967 &  0.88847 &  0.88106 &  0.87363 &  0.87015 &  0.86320 &  0.86221 &  0.86109 &  0.86088 \\
    210          &  0.91967 &  0.89970 &  0.88769 &  0.87966 &  0.87184 &  0.86772 &  0.86179 &  0.86061 &  \textcolor{blue}{0.85979} &  0.85980 \\
    \bottomrule
    \end{tabular}
    \caption{IE Loss}
    \label{tab:my_label}
\end{table}


==> tables/table_bootstrap.tex <==
\begin{table}[H]
    \caption{Results on bootstrap semi-synthetic data. Reported performance metrics are averaged over $30$ runs. }
    \centering
    \begin{tabular}{|p{3.3cm}||p{2.1cm}|p{1.8cm}|p{1.8cm}|}
         \hline
         Model &  $\qadj~(\mathrm{S.E.})$ & $\hat{v}~(\mathrm{S.E.})$ & $\hat{\mathcal{R}}~(\mathrm{S.E.})$\\
         \hline
    %TRAIN
         \multicolumn{4}{|c|}{Training Set ($n=7,000$, $p=40$)} \\
         \hline
         Qini-based UR  &  & & \\
         Causal Forest  &  & & \\
         Causal Forest (H) &  & & \\
         Random Forest (ED) &  & & \\
         Random Forest (KL) &  & & \\
         SMITE (TO) &  & & \\
         SMITE (IE) &  & & \\
         \hline
    %VALID
         \multicolumn{4}{|c|}{Validation Set ($n=3,000$, $p=40$)} \\
         \hline
         Qini-based UR  &  & & \\
         Causal Forest  &  & & \\
         Causal Forest (H) &  & & \\
         Random Forest (ED) &  & & \\
         Random Forest (KL) &  & & \\
         SMITE (TO) &  & & \\
         SMITE (IE) &  & & \\
         \hline
    \end{tabular}
    \label{tab:boot_perf}
\end{table}

==> tables/table_real_data.tex <==
\begin{table}[H]
    \caption{Results on Canadian insurance dataset. Reported performance metrics are averaged over $30$ runs. }
    %For both statistics, the higher is better. On the other hand, overfitting can be assessed by the difference in magnitudes between training set and out-of-sample set.
    \centering
    \begin{tabular}{|p{3.3cm}||p{2.1cm}|p{1.8cm}|p{1.8cm}|}
         \hline
         Model &  $\qadj~(\mathrm{S.E.})$ & $\hat{v}~(\mathrm{S.E.})$ & $\hat{\mathcal{R}}~(\mathrm{S.E.})$\\
         \hline
    %TRAIN
         \multicolumn{4}{|c|}{Training Set ($n=21,000$, $p=40$)} \\
         \hline
         Qini-based UR  &  & & \\
         Causal Forest  &  & & \\
         Causal Forest (H) &  & & \\
         Random Forest (ED) &  & & \\
         Random Forest (KL) &  & & \\
         SMITE (TO) &  & & \\
         SMITE (IE) &  & & \\
         \hline
    %VALID
         \multicolumn{4}{|c|}{Validation Set ($n=14,000$, $p=40$)} \\
         \hline
         Qini-based UR  &  & & \\
         Causal Forest  &  & & \\
         Causal Forest (H) &  & & \\
         Random Forest (ED) &  & & \\
         Random Forest (KL) &  & & \\
         SMITE (TO) &  & & \\
         SMITE (IE) &  & & \\
         \hline
    %TEST
         \multicolumn{4}{|c|}{Out-of-sample ($n=15,000$, $p=40$)} \\
         \hline
         Qini-based UR  &  & & \\
         Causal Forest  &  & & \\
         Causal Forest (H) &  & & \\
         Random Forest (ED) &  & & \\
         Random Forest (KL) &  & & \\
         SMITE (TO) &  & & \\
         SMITE (IE) &  & & \\
         \hline
    \end{tabular}
        \label{tab:realdata_perf}
\end{table}

==> tables/table_synthetic.tex <==
\begin{table}[H]
     \caption{Results on synthetic data. Reported performance metrics are averaged over $30$ runs. }
    \centering
    \begin{tabular}{|p{3.3cm}||p{2.1cm}|p{1.8cm}|p{1.8cm}|}
         \hline
         Model &  $\qadj~(\mathrm{S.E.})$ & $\hat{v}~(\mathrm{S.E.})$ & $\hat{\mathcal{R}}~(\mathrm{S.E.})$\\
         \hline
    %TRAIN
         \multicolumn{4}{|c|}{Training Set ($n=7,000$, $p=40$)} \\
         \hline
         Qini-based UR  &  & & \\
         Causal Forest  &  & & \\
         Causal Forest (H) &  & & \\
         Random Forest (ED) &  & & \\
         Random Forest (KL) &  & & \\
         SMITE (TO) &  & & \\
         SMITE (IE) &  & & \\
         \hline
    %VALID
         \multicolumn{4}{|c|}{Validation Set ($n=3,000$, $p=40$)} \\
         \hline
         Qini-based UR  &  & & \\
         Causal Forest  &  & & \\
         Causal Forest (H) &  & & \\
         Random Forest (ED) &  & & \\
         Random Forest (KL) &  & & \\
         SMITE (TO) &  & & \\
         SMITE (IE) &  & & \\
         \hline
    \end{tabular}
    \label{tab:synthe_perf}
\end{table}
